A Guide to Evaluating the Experience of Media and Arts Technology

Evaluation is essential to understanding the value that digital creativity brings to people's experience, for example in terms of their enjoyment, creativity, and engagement. There is a substantial body of research on how to design and evaluate interactive arts and digital creativity applications. There is also extensive Human-Computer Interaction (HCI) literature on how to evaluate user interfaces and user experiences. However, it can be difficult for artists, practitioners, and researchers to navigate such a broad and disparate collection of materials when considering how to evaluate technology they create that is at the intersection of art and interaction. This chapter provides a guide to designing robust user studies of creative applications at the intersection of art, technology and interaction, which we refer to as Media and Arts Technology (MAT). We break MAT studies down into two main kinds: proof-of-concept and comparative studies. As MAT studies are exploratory in nature, their evaluation requires the collection and analysis of both qualitative data such as free text questionnaire responses, interviews, and observations, and also quantitative data such as questionnaires, number of interactions, and length of time spent interacting. This chapter draws on over 15 years of experience of designing and evaluating novel interactive systems to provide a concrete template on how to structure a study to evaluate MATs that is both rigorous and repeatable, and how to report study results that are publishable and accessible to a wide readership in art and science communities alike.

==> sections/03_Analysis.tex <==
\section{Analysing Data}
\label{ch:analysis}

There are many ways to assess data depending on the type of data you have collected and the questions you are asking in your study. In general, you will want to analyse your data focusing on the specific research questions you have come up with; this will help you to choose the correct analysis and to plan a clear and concise study.

First, we will go through the types of statistical tests and how statistical analysis can be used to get a clear picture of quantitative data. Then, we will discuss qualitative analysis, namely Thematic Analysis, for other types of data collected.

When deciding what kind of test to do, besides the difference between quantitative and qualitative data, you should also consider: 
\begin{itemize}
    \item The number of participants you have
    \item The structure of the study (e.g., repeated or unrepeated measures)
    \item The kind of data you collected (e.g., nominal, ordinal, interval, or ratio)
\end{itemize}

\subsection{Statistical Analysis}
Statistical analysis is used with quantitative data to assess whether the results we have observed match our hypothesis or not. In this sense, it is very important to have specific hypotheses mapped out in your study design so that you can appropriately collect data and choose a statistical method to test it! We use statistical tests to determine whether there are significant relationships between variables or difference between groups. By significant here we mean that the differences are not likely to be just due to chance. 

A statistical analysis involves running one or more statistical tests on your data. Each type of statistical analysis involves a number of assumptions and considerations, so it is usually a good idea to be familiar with the tests and what is needed to conduct them. You cannot just perform a test without checking these assumptions or meeting criteria, as you will likely get incorrect results. 

\subsubsection{Checking Data Assumptions}
Statistical tests are either parametric or non-parametric. You will need to decide whether you use a parametric or non-parametric stats test depending on your data. Parametric tests are more powerful but usually can only be used with interval and ratio data. In order to use a parametric test, your data must have independent observations, homogeneity of variance, and be normally distributed. Non-parametric tests do not assume normal distribution of data (often converting data into rankings), so they can be used with ordinal, interval, and ratio data, and data which is not normally distributed. However, they are less powerful, so you need to have an explanation why you could not use a parametric test.

\subsubsection{Data Transforms}
Often, the dependent variable data can be transformed so that it meets a normal distribution and variance. Data often have a natural skew which can be evened through transformation. You can plot a histogram of your data/groups to see how the distribution falls. Some of the most common transforms you can use are log, square root, or cube root transforms. 

\subsubsection{Types of Statistical Test}
Once you know whether your data is parametric (before or after transformation) or not, you can select a statistical test to check your hypotheses. Some kinds of test are ONLY parametric, but there are non-parametric equivalents for most tests.
There are three main types of parametric test: regression, comparison, and correlation tests:

\begin{enumerate}
    \item \textbf{Regression} – checks to see a cause-and-effect relationship between continuous independent variables and outcomes (e.g., the relationship between the number of minutes spent training on a MAT and the rhythmic complexity measurement of the resulting song). Predictors are continuous.
    \item \textbf{Comparison} – checks differences between group means to see if the groups are different or similar (e.g., checking to see whether non-musicians or musicians make more annotations during a listening test). Predictors are categorical.
    \item \textbf{Correlation} – checks whether variables are related (not necessarily a cause-effect relationship as in a regression, e.g., how are years of musical theory training and rating of a MAT related?)
\end{enumerate}

\subsubsection{Repeated-Measures Testing}
As mentioned earlier, it may sometimes be useful to have participants perform more than one task during a study or to interact with different conditions. These are still independent observations because the conditions are different (e.g., the data is still parametric), but we must perform alternative statistical tests because the participants were tested more than once. Fortunately, the majority of statistical tests can be used for repeated measures.

For example, the Repeated Measures ANOVA is a common test used in statistical analysis. When running the repeated measures test, the related groups (eg, the participants who were tested more than once) are measured instead of the individual groups. You compare the measurement of the same result between conditions instead of between participants. In this case, you may also see the independent variable called the within-subjects factor. For example, if you are testing usage of a MAT over time (eg. at two-weeks, 1-month, and 3-months of use), you would compare each participant’s usage at the three conditions (time).

\subsubsection{Sample Size}
Another point to consider when selecting a statistical test is sample size. Statistical power is important in considering the results of your statistical test. If too few participants are used for the test, given the number of variables or conditions examined, the results may be incorrect or unclear. It is extremely beneficial to determine an appropriate sample size when designing your study and determining the tests you want to perform on the data. This will help to make sure you will be able to gather enough participants for the tests you want to do.

In general, you will need at least 10 participants in a proof-of-concept study. For a comparative study you need at least 10 participants for each condition. As well, you can calculate the statistical power of the tests you want to run with your expected sample size. \href{ https://www.psychologie.hhu.de/arbeitsgruppen/allgemeine-psychologie-und-arbeitspsychologie/gpower.html}{G*Power} is a common tool used to assess statistical power and necessary sample sizes and can give you a good estimate of the number of participants you will need to use different statistical tests given your study parameters.

\newpage
\subsubsection{Choosing a Statistical Test}
Depending on your predictor and outcome variables and whether or not your data is parametric, you will need to select the most appropriate statistical test. You can reference the above tables to determine which test is appropriate given your independent predictor variables and your dependent outcome variables. Additionally, the following flow chart (A Painless Guide to Statistics, Dr. Robert Gerwien) can be used to help you decide:
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.87\textwidth]{figures/statsflowchart}
    \caption{Flow chart for selecting commonly used statistical tests (Gerwien, A Painless Guide to Statistics).}
    \label{fig:flowchart}
\end{figure}

\subsubsection{Post-hoc Testing}
Additionally, if you use statistical tests which handle two or more categories (e.g., ANOVAs), you will need to run some post-hoc tests to determine which specific categories are different. This is done in the form of pairwise comparison tests. If you find that there is a significant difference in the data set, then you can do multiple pairwise comparisons. Note that stats people insist that you must check the whole data set first to check for overall significance BEFORE you do the pairwise comparisons.

For example, if are testing the effect of three interfaces, A, B and C, on an output variable, you will initially do an ANOVA to determine if there is a significant effect of interface on that output. If that test is significant, you know that there is an effect; however, you cannot say whether A, B, or C are causing this effect. Pairwise comparisons will allow you to look at interfaces in pairs (hence the name) to determine where the differences are – between A and B, B and C, and A and C. 

Pairwise comparisons are typically Bonferroni-adjusted (there are other adjustment types, but this is the most common). Because you are doing multiple tests, the expected probability levels also change and therefore the p-value estimation also needs to be adjusted. Typically, statistics software will automatically conduct Bonferroni-adjusted pairwise comparisons when the comparisons are calculated.

\subsubsection{Reporting Stat Test Results}
Depending on which format your publication is in, the presentation of statistical results will be slightly different, but generally follow the same formats. The reporting guidelines here are all correct for APA formatting.

\paragraph{The p-value}
The most important statistical measure in reporting (there is some debate about p-values being viewed as the end-all-be-all in results reporting, so it is important to use critical thinking about your analyses and interpret the p-value in an appropriate way), the p-value is the probability that the result or was due to chance. In HCI, we usually consider something to be statistically significant if the $p$ is less than .05 ($p < .05$)\footnote{NB: In APA formatting, you should not include a leading 0 when reporting p-values because they exist only between 0 and 1.}. You will also see other p-values of $< .01$ and $< .001$ – these are not typically used in HCI research (see below for more information on the confidence interval).

\subsubsection{Additional Terminology}
There is some additional terminology you may encounter when reading others’ work or presenting your own statistical analyses. Although it is not necessary to fully understand these stats concepts to do your own basic analyses, it is good to have a basic knowledge of these concepts.

\paragraph{Confidence Intervals}
A confidence interval (CI) gives a range of values that we are sure the true result value lies within. Typically, we use CI to express a range for mean or standard deviation in a population. With a CI 95\%, we are fairly confident that the true value is observed in this experiment. This does mean that there is a 5\% chance the experiment does not include the true value; there is still a small chance that what we observed in the experiment is due to chance. However, in HCI we deem this probability to be acceptable and that it is likely that other experiments will return the same result to our experiment. 

\paragraph{The Null Hypothesis}
When you are conducting statistical tests or reporting them, you may see mention of the null hypothesis. It was previously mentioned that statistical tests check the probability that what you observed in your study was due simply to chance; in fact, statistical tests check the probability of the null hypothesis. The null hypothesis usually states the contrary or opposite of your hypothesis; for instance, if you hypothesise that musicians will have different reactions to an aspect of your interface than non-musicians, the null hypothesis will state that there is no difference between the musicians and non-musicians. Null hypotheses, aptly named, are null – there is no relationship between the variables, no correlation, no differences between groups, etc. When you do a statistical test, you check the likelihood of the null hypothesis, which is why we want our p-values to be so small. We want to be sure that the confidence interval does not include the null value. A small p-value means there is a small probability that the null hypothesis is true (and our examined hypothesis is likely). For example, if a paired t-test examining the difference between before- and after-training usage time on an interface returns a p value of .03, we can conclude the null hypothesis is unlikely and therefore there is a difference between usage time before and after training.

\subsection{Thematic Analysis}\label{sec:ta}
When analysing qualitative data, Thematic Analysis (TA) is a useful method for robust and systematic review. TA can be used for interview data, questionnaire responses, video data, and other types of open-ended feedback. Through TA, we can identify key patterns of meaning (themes) in the data. In general, TA works through identification of key points in a data set, called codes, which are then organised into larger, overarching themes.

\subsubsection{Types of Thematic Analysis}
There are several kinds of TA which can be used to examine qualitative data. The two most common types you will encounter or expect to use are:

\begin{itemize}
    \item Deductive: the coding and themes are dependent on existing concepts or ideas about the data (e.g., from previous research)
    \item Inductive: the coding of the data and resultant themes are a result of the data content and emergent patterns.
\end{itemize}

If you expect to observe some kind of pattern in your data, it may be helpful to use a deductive approach. For instance, in the Daisyphone research, the interface was informed by existing CSCW work which that sense of identity is important in collaboration; therefore, in examining participant feedback during TA, it may be useful to deduce codes and themes which are related to this existing knowledge. The focus of the TA may be on comments about ownership or collaboration, or the reaction of participants to the colour features of the interface.

In more exploratory studies, it can be helpful to take an inductive approach. In this sense, the analysis is done in more of an open or exploratory way. Through reviewing the data, the researcher may notice different emergent codes and similarities, which then become themes. This is often a good way to explore participant interactions or post-study feedback, as inductive TA can reveal patterns which are unexpected or aspects of interaction which may not have been considered previously. In following studies, these observations can then be used as the focus for study design.

\subsubsection{Phases of Thematic Analysis}
Because there is no set way to perform TA, the steps can be done in a flexible way depending on the knowledge of the data and the specific questions being explored. On the other hand, in order to perform a robust review, it is important to document all of the steps of TA, including coding and changes made over time, and how and why resultant themes were organised in the final version of the analysis.

Generally, TA is conducted as such:
\begin{enumerate}
    \item \textbf{Data review}: Familiarising yourself with the data. This involves reading and re-reading and re-re-reading the data to become familiar with it.
    \begin{itemize}
        \item As you read through the data, you will begin to see similarities or important points. It is good to make a note of these as you go through.
        \item Reviewing video data and listening to recordings can also be helpful in picking up other semantic cues from participants (e.g., tone of voice, laughter, other emotion in addition to the word content)
    \end{itemize}
    \item \textbf{Initial Coding}: In an additional read-through of the data, begin to generate codes of important data features you identify. 
    \begin{itemize}
        \item Codes should be succinct, single points or sentences in the feedback.
        \item This should be done iteratively - read-through the entire data set and generate codes, then begin again and find any connections which may have been missed, or further refine the codes.
    \end{itemize}
    \item \textbf{Generate Initial Themes}: From the set of codes, begin to organise them into overarching themes
    \begin{itemize}
        \item These themes should be descriptive and provide a clear relationship between the codes
        \item It is okay if a code fits into more than one theme - overlap between ideas is natural; however, if there are many overlaps between two themes it might be more suitable to unite them into a single theme
    \end{itemize}
    \item \textbf{Review \& Refine}: As you begin to organise the themes, you may remove codes and themes, re-code material, or add additional codes and themes.
    \begin{itemize}
        \item The process is meant to be iterative - it is normal and appropriate to make informed changes as you review the material and make more connections between the codes and themes.
        \item Keep a note of how the codes/themes change over time, as it will be helpful in generating the final descriptions of the themes.
    \end{itemize}
    \item \textbf{Define Final Themes}: Once you are satisfied the coding and theme organisation paints a clear picture of the data, determine the `story' of each theme, how it plays a role in what was observed during the study, and what the patterns encompassed in it are.
    \begin{itemize}
        \item You should come up with clear, concise, and informative names for your themes at this stage.
        \item As you come up with a clear definition for the theme, you may find that some themes can be consolidated; be sure to justify how each theme is distinctive.
    \end{itemize}
\end{enumerate}

As the process is iterative, it is important to plan effectively and to remember that TA typically takes longer than you might anticipate. It is common to spend a few weeks getting to know the data well and going through the processes of coding and re-coding. Additionally, it is helpful to take some time in between coding sessions to process the data effectively.

The themes generated will contain a number of codes and references from the data set. It is important to remember that TA is meant to provide a story of the data; therefore, a theme may still be critical even if it is only referenced a few times. If the theme provides an important perspective to the overall narrative of the data, it is worth including and justifying its relevance.

For instance, in a study examining underlying reasons for different emotion perception in live music performance \citep{yang:2021}, participants were asked to include long-form feedback on why they annotated emotion changes at different points in the data. Of the 1255 codes generated in review of this data, 2 codes included participant responses related to the lighting and visuals on stage as being the cause of their emotion perception; although this is a small percentage of the overall codes, it still highlights an important factor in live music performance. The resultant theme for these two codes, \textit{Stage and Visuals} provides important insight that environmental factors provide emotional cues: ``Even in a lab
viewing of performance video, participants were able to associate emotion with changes in stage lighting, underscoring
the relevance of environment on perception.'' 

\paragraph{Quotes from Participants}
It is important to provide quotes from participants in your TA results and also when reporting the results of questionnaires and interviews. This provides evidence that you have objectively collected opinions about your MAT. As well, referencing specific data points/codes when describing a theme can help to better contextualise the material and the meaning of the theme. When referencing specific points, include the participant's ID number.

Quotes should be short and concise to support specific points, only choosing the relevant portion of the feedback, e.g., if a participant said or wrote in their response: ``Well, I enjoyed the experience a lot and found it quite engaging. I was thinking about it the other day whilst walking to work and thought that it was quite nice. That is just my opinion of course, but in general that is my feeling about it. Yes.'' (P2), you should not quote the whole paragraph, but instead quote the key points, e.g., ``I enjoyed the experience a lot and found it quite engaging'' (P2). The other points are just repeating this point. If you are really short of space, you can reduce it further, e.g., ``enjoyed the experience a lot... quite engaging'' (P2).

Make sure to include a range of participants’ responses – don’t just report one or two participants. If you have 5 participants, make sure to provide quotes from each of them in your results. If you have more than 5 participants then try to report a balance of responses – positive as well as negative. Remember that negative responses are still useful in terms of research, and give you something interesting to discuss in your discussion section – i.e. why do you think that they gave negative responses etc.?

For a PhD thesis you would include the full transcripts of interviews and all the questionnaire answers in your Appendix.

\paragraph{Reporting Thematic Analysis Results}
When reporting your Thematic Analysis, make sure in the methods to include which kind of TA you conducted (either deductive or inductive). Additionally, if you transcribed audio or video data, it is useful to include the level of detail which was transcribed and analysed (e.g., did you include non-verbal utterances such as laughter, facial expressions, etc.).

\begin{wrapfigure}{r}{0.47\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{taYang} 
\caption{A table presenting main themes and relevant codes, adapted from \citep{yang:2021}).}
\label{fig:TAtable}
\end{wrapfigure}

Report how many codes you developed in the TA and provide a general overview of the themes (you do not need to list the codes, but this may be helpful in getting a clearer view of the data). List the themes that you identified in the TA. Should should list the number of codes within each theme. However, remember that the number of codes within a theme does not dictate relevance; the themes are meant to create a clear picture of the data and capture important points and similarities. If the theme contains only one or two codes but provides a critical observation from the research, it is still a valid theme.

E.g. “Overall, 39 codes were identified in the Thematic Analysis of the interviews, leading to six broad themes: (i) Design process (10 codes); (ii) co-creation (8 codes); (iii) interactivity (6 codes); (iv) translation (4); (v) drama style (4); and (vi) role of local context (7 codes).” \citep{bryankinns:2018}.

Additionally, you may find it is helpful to include a table of themes and relevant codes for a reader to reference easily. For example, the table adapted from \citep{yang:2021}. (Figure \ref{fig:TAtable}).

Then provide a description of each of the themes. The description is usually at least a couple of sentences, and if you have space it could be several paragraphs. In the description make sure to illustrate your description with quotes from participants and refer to the participant ID. Remember that TA is about providing a cohesive picture of the data from the codes, so the themes should be linked together and discussed thoroughly.

E.g. “Theme: Design process. In the interviews team members reported that during the Qi2He process most of the creative decisions were made by the participants together… though from the interviews it is clear that not all of the elements were contributed to equally by the groups… Local musicians did not comment on the design process as being novel. P1 commented that the ‘whole process matches his former experience of working with local singers’, and that because there is no new music, he didn’t see that he was doing co-creation work” (adapted from Bryan-Kinns et al., 2018).

It is also appropriate to connect themes and descriptions to existing work in order to highlight relevance. For example, in the Stage and Visuals theme \citep{yang:2021}:

``Two reactions were derived from visual reference, although there was no instruction in the task to examine beyond the music in the audio-video recording. Both refer to stage lighting; in particular, participants associated the decrease of arousal with the lights darkened in the final segment: ``The violin changes the length of the notes and with that the energy of the music. Also as it does not have light it is less energy as in the other parts.'' - P21, S17 (11:47). Although this is not a frequently occurring theme, it does highlight the impact of context and setting. Even in a lab viewing of performance video, participants were able to associate emotion with changes in stage lighting, underscoring the relevance of environment on perception. As emotion contagion means members of an audience are likely to react in similar ways to their fellow concert-goers (Goffman, 1964; Fridlund, 1991), it is worth exploring the impact of environment, staging, and venue on the perceived emotion content for a performance.''

==> sections/04_Reporting-Reslts.tex <==
\section{Reporting MAT Studies}
\label{ch:report}

When reporting your results, either in a presentation or paper, you should reference the structure defined in Section \ref{ch:methods} and include the sections outlined there. In general, research findings begin with an Abstract, followed by Introduction, Methodology, Results, Discussion, and finally a Conclusion.

\subsection{Abstract}
The Abstract is a short summary of your study and the findings. Although it is the first part of a paper, it is often easier to write the abstract after you have written everything else, in order to get a concise summary of the contents of the presented research. An abstract is usually 250 words (often shorter). Make sure to highlight the key contributions of the paper, so that a reader will know what to expect. This is also important in the peer review process, so an editor can appropriately assign a reviewer for your work. 

\subsection{Introduction}
The Introduction presents the research topic and what is being explored in the study. The Introduction is an expansion of the Abstract and provides a high-level explanation of the work and why the study is being done. The Introduction can be used as an outline for the presentation, telling a reader what the rest of the paper will comprise of and what the key findings of the paper are.

\subsection{Background}
The Background researched at the beginning of the study design should be presented here to provide context for the reader. The related work should present the state-of-the-art and identify gaps in the existing knowledge which are explored in the current work. Many authors use the final paragraph of their Background section to list their research aims, study questions, and/or hypotheses tested, highlighting the novelty of the study and setting up expectations for the readers. 

\subsection{Methodology}
Methodology is important in order to ensure the study is robust and reproducible, as discussed in Section \ref{ch:methods}. The methodology should include detailed information about the procedure so that another researcher may reproduce it exactly. You may find it helpful to include subsections for each component mentioned in Section \ref{ch:methods}.

An example of the specificity in the Methods section of \citep{yang:2021}: ``Participants annotated on a 13” MacBook Air in a sound proof listening studio at QMUL. Audio stimuli were presented through headphones (Beyerdynamic DT 770 Pro) and video on the laptop display.''

The Methodology should include all of the information about how the study was conducted, including the variables and conditions examined, the tools used including existing materials (e.g., questionnaires used) or technology created for the study (e.g., your MAT), and how the data was collected. 

\subsubsection{Participants}
In your Methodology, you must describe your participants in detail, including how many participants took part in the study, how they were recruited, 
whether they were paid an incentive, and give some demographic information about the participants, such as age (range, mean, and standard deviation), gender, nationality distribution, and background material collected through relevant questionnaires, such as the Gold-MSI.

For example, in \citep{bryankinns:2009} we said:

``Final year Computer Science students at the first author's institution were recruited through advertisements to take part in the experiment as part of their course, but not offered any incentives to take part. Thirty-nine of a possible 80 participants took part (28 males, 11 females; aged from: 20 to 29; mean age: 22, average computer literacy: expert; average musical ability: intermediate; none were professional or trained musicians; none had used Daisyphone before). Participants’ musical preferences ranged from Hip Hop (most popular) to Latin (least popular).''

If you report individual responses in your results (e.g., interview answers), then you should give a table to provide brief demographic of each participant, as this may have an impact on their answers. Give each person a participant ID (e.g. P1, P2, etc.) which you can then use in the results. For example, see Table \ref{tab:pttable}. 

\begin{table}[ht]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Participant} & \textbf{Age} & \textbf{Gender} & \textbf{Musical ability} & \textbf{Musical preference} \\ \midrule
P1                   & 25           & M               & Novice                   & Hip hop                     \\
P2                   & 24           & M               & Intermediate             & Hip hop                     \\
P3                   & 20           & F               & Intermediate             & Hip hop                     \\
P4                   & 22           & M               & Intermediate             & Rock                        \\
P5                   & 21           & F               & Expert                   & Latin                       \\
P6                   & 22           & M               & Novice                   & Classical                   \\
P7                   & 22           & M               & Intermediate             & Rock                        \\
P8                   & 21           & F               & Intermediate             & Ambient                     \\ \bottomrule
\end{tabular}
\caption{Example table for presentation of participant demographics and background.}
\label{tab:pttable}
\end{table}

\subsubsection{Analyses}
Analyses should be presented referencing the specific method used. This section should only include how the Analyses were conducted, saving the results until the subsequent Results section. 

Here, it is important to describe different measures taken from the data; for instance, how participant involvement was measured, how musical complexity was determined, and so on. Additionally, this is an ideal place to discuss why different analysis methods were were chosen; for instance, justifying the choice of a statistical test.

\subsection{Results}
Results should be presented based on the types of analyses done, as outlined in Section \ref{ch:analysis}. If you performed multiple analyses, for instance a statistical analysis of study outcomes and then a Thematic Analysis of participant feedback, the results section should be divided into separate parts.

\subsubsection{Other Observations}
It may be beneficial to provide other observations made during the study which do not fall into a specific category of analysis. Provide vignettes of observations that support or illustrate findings from your other data. Vignettes are short descriptions of some action and interaction and would often be accompanied by an image from your video recording if you have it.

E.g., from \citep{bengler:2013}:
``A prevalent input strategy was the creation of musical patterns characterised by simple geometric properties. The most common phrases consisted of horizontal and upward or downward diagonal lines whereas in most cases all available notes were used (Figure \ref{fig:contributions}). Resulting in ‘closed musical figures,’ this approach was applied by many players providing a clear audio-visual correlation between the representation on the interface and the musical result.''

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/contributions.png}
    \caption{A vignette of typical contributions.}
    \label{fig:contributions}
\end{figure}

\subsubsection{Questionnaire Results}
Generally, when reporting questionnaire results, you want to report either a data count or a range-mean-standard deviation set. The report depends on the kind of data. For nominal and ordinal data, you will generally want to report a count; for example, ``All participants indicated the interface was Enjoyable (18 participants) or Very Enjoyable (30 participants) to use.'' For interval and ratio data, you will want to include the range of the response, the mean, and the standard deviation; for instance, ``Participants reported that they used the new interface for a longer duration of time, ranging between 45-65 minutes (M = 50, SD = 2.5).''

You can visually report the results of Likert scale questions using a box-and-whisker plot. These are good at showing many aspects of your data – they show the minimum, the maximum, the median, the upper quartile (top 75\%) and lower quartile (lower 25\%) of your results. For example, the box-and-whisker plot in Figure \ref{fig:box} shows responses given for elements of playing experience \citep{bengler:2013}. Note the clear labelling of the x and y axes -- make sure to clearly label your graphs.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/box.png}
    \caption{Example results presentation using a box-and-whisker plot (adapted from \citep{bengler:2013}).}
    \label{fig:box}
\end{figure}

\subsection{Discussion}
In the Discussion, you should reflect on your results -- what results were unexpected, why do you think that might be? What explanations can you think of for the results you found? Connect your results back to the Background and the aims of your study -- did your results match with the results of other researchers you mentioned in the literature review? If not, why not? What do your results tell you about the things you wanted to find out in the aims of your study?

It is quite usual to find things that you did not expect, or which are surprising and counter intuitive. This is part of why we conduct these exploratory MAT studies. The Discussion can explore why the results were unexpected and suggest future work to further explore the findings in future work (hopefully using your well-reported and rigorous methods). The most important thing is to clearly and objectively report the results, and then reflect on your results, connecting them to your literature review, your study aims, and your intuition about what happened.

\subsubsection{Limitations}
This is also the place to discuss limitations to your research. In terms of \textit{internal} and \textit{external validity}. Ideally, your research will have both; in the case it does not, you will need to highlight where the reported results are limited.

Internal validity is the extent to which the study accurately and confidently depicts the relationship between the variables being examined. Some factors which might influence the internal validity are uncontrolled or confounding variables, small sample size, repeated testing and learning effects and potential experimenter bias.

External validity refers to the the extent that the findings of the study can be applied in other settings -- how generalisable the findings are to the world outside of the study. Some factors which might reduce the external validity are selection bias (e.g., the participants who take part in a MAT study might be interested in/already using technology in artistic settings, so might react differently than others who are not as likely to participate), situational factors such as time of day and location, and limited examined factors, such as only looking at music within the Western canon.

In either case, you must identify these factors in validity, not only to lead future work but also to demonstrate your awareness and acknowledgement of potential limitations in the work. For instance, in \citep{yang:2021}, only a singular piece of music was examined during the study. It was therefore necessary to note that there is some limitation to the external validity and that further study is required: 

``Although the Babajanian Trio is well situated within the Western contemporary music canon and spans a wide range of characteristics, the findings drawn from this recording cannot be generalised to other music without further study.''

\subsubsection{Future Work}
After providing the results and having discussed some limitations, it is worthwhile to suggest future research studies which will further explore the results you have achieved or address the limitations. You might also include some suggestions for research based on interesting or exciting findings, to expand or apply what was learned through the study to additional research questions.

\subsection{Conclusion}
Finally, after you have finished your discussion, you should include a Conclusion section to summarise the study and your relevant findings. This should tie together the components of the study and highlight the main takeaways for the reader.
